A New Family of Neural Networks Provably Resistant to Adversarial Attacks

Adversarial attacks add perturbations to the input features with the intent of changing the classification produced by a machine learning system. Small perturbations can yield adversarial examples which are misclassified despite being virtually indistinguishable from the unperturbed input. Classifiers trained with standard neural network techniques are highly susceptible to adversarial examples, allowing an adversary to create misclassifications of their choice. We introduce a new type of network unit, called MWD (max of weighed distance) units that have a built-in resistant to adversarial attacks. These units are highly non-linear, and we develop the techniques needed to effectively train them. We show that simple interval techniques for propagating perturbation effects through the network enables the efficient computation of robustness (i.e., accuracy guarantees) for MWD networks under any perturbations, including adversarial attacks. MWD networks are significantly more robust to input perturbations than ReLU networks. On permutation invariant MNIST, when test examples can be perturbed by 20% of the input range, MWD networks provably retain accuracy above 83%, while the accuracy of ReLU networks drops below 5%. The provable accuracy of MWD networks is superior even to the observed accuracy of ReLU networks trained with the help of adversarial examples. In the absence of adversarial attacks, MWD networks match the performance of sigmoid networks, and have accuracy only slightly below that of ReLU networks.

==> bounds.tex <==
\newcommand{\bx}{\vecx}
\newcommand{\bu}{\vecu}
\newcommand{\bw}{\vecw}
\newcommand{\beps}{\mathbf{\epsilon}}

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}

\section{Accuracy Lower Bounds For Adversarial Attacks}
\label{sec-bounds}
For an arbitrary network $\cal N$, and input $\vecx$, we provide a technique for estimating the maximum output perturbation that can be obtained by perturbing the input by at most $\epsilon$. 
Our technique calculates an input-dependent sensitivity by computing the range of values that can be produced at each node under a given amount of input perturbation, 
and is efficient for a wide variety of node types, including sigmoid, ReLU, and MWD.

\paragraph{Definitions.}
The \emph{$\epsilon$-perturbation} of an input $\vecx$ is any $\vecx'$ where $|| \vecx - \vecx' ||_\infty \leq \epsilon$ and the input belongs to the input domain. 
Given a classifier, an \emph{$\epsilon$-adversarial example} for input $\vecx$ is an $\epsilon$-perturbation of $\vecx$ that results in a different prediction.
The \emph{true $\epsilon$-attack accuracy} of a trained network is the fraction of test examples for which the network predicts correctly and no $\epsilon$-adversarial examples exist.

\smallskip 

Since adversarial examples are often hard to find, this true attack accuracy is difficult to measure.
Given a particular heuristic for producing $\epsilon$-attacks, we can measure the fraction of examples in the testing set that are predicted correctly, and for which the heuristics is unable to find an $\epsilon$-adversarial example. 
Each heuristic (or attack strategy) yields an upper bound on the true $\epsilon$-attack accuracy of the network.
Unfortunately, determining whether there exists an $\epsilon$-perturbation that causes a misclassification (and thus, determining the true $\epsilon$-attack accuracy) is NP-complete, as the following theorem shows.
The theorem is a somewhat unsurprising consequence of the relationship between neural networks and boolean circuits.

\begin{theorem}
Given a MWD network, input $\vecx$ and output $\vecy$, deciding whether there is an $\epsilon$-perturbation of $\vecx$ that yields output $\vecy$ is NP-complete. 
\end{theorem}

\noindent {\em Proof (sketch).}
The existence of polynomial-time witnesses shows that the problem is in NP.
The proof consists of a reduction from 3-SAT \cite{GareyJohnson}. 
Consider a set of predicate letters $P = \set{p_1, \ldots, p_n}$, their complements $\bar{P} = \set{\bar{p}_1, \ldots, \bar{p}_n}$, and a set $C = \set{c_1, \ldots, c_m}$ of clauses, with $c_j \subs P \union \bar{P}$ for $1 \leq j \leq m$. 
% We will construct a network whether a given output can be reached by a 0.5-perturbation of the input only if the 3-SAT problem is satisfiable. 

Given an instance $C$ of 3-SAT, we construct a network with two layers.
We can show that the problem is NP-hard already for $\vecx = \tuple{0.5, \ldots, 0.5}$ and $\epsilon=0.5$ (the theorem can be strengthened to hold for specific $\epsilon$-values).
In the first layer, there is one unit $N^{(1)}_j$ for each clause $c_j$.
If $p_i \in c_j$, then we set $w^{(1)}_{ji} = 0$ and $u^{(1)}_{ji} = 1$; 
if $\bar{p}_i \in c_j$, we set $w^{(1)}_{ji} = 1$ and $u^{(1)}_{ji} = 1$; 
we set $w^{(1)}_{ji} = u^{(1)}_{ji} = 0$ otherwise. 
If the network inputs can be only either 0 or 1, the output $z_j$ of $N^{(1)}_j$ can reach $1/e$ only if $c_j$ is satisfied. 
In the second layer, there is only one unit, with one input for each clause.
For this unit, we set $w^{(2)}_j = 1/e$ and $u^{(2)}_j = 1$ for each input $j$ (from $N^{(j)}$); the output $y$ of this layer can reach $1$ only if every $z_i$ is $1/e$. 

It is not difficult to see that the network yields output $1$ for an $0.5$-perturbation of the input $\vecx = \tuple{0.5, 0.5, \ldots, 0.5}$ iff the 3-SAT instance is satisfiable.
\qed

\smallskip 

It is not too difficult to generalize this result to show that (for any $1\leq \epsilon>0$) the problem of given a MWD network, input $\vecx$, and output node $j$, determining if 
an $\epsilon$-perturbation of $\vecx$ exists that causes node $j$ to output the midpoint of its perturbation interval is NP-complete.
\citet{weng18a} show related hardness results for approximating the range of outputs produced by $\epsilon$-perturbations in ReLU networks.

\newcommand{\perb}[1]{{I}_{#1}^\epsilon}
\newcommand{\perbj}{\perb{j}}

In view of this hardness result, we present an approximate technique which propagates  {\em perturbation intervals\/} forward through the network.
These over-approximate the actual range of values that the outputs of the nodes can attain when a particular input example is subject to perturbations.
Like the approach of \citet{wong18a}, we calculate a convex approximation to the set of layer outputs that can be produced by an $\epsilon$-perturbation.
Their approach can handle different perturbation norms but is specialized for ReLU networks, while our simpler method easily generalizes to different node types.


% This will yield efficiently computable lower bounds for the true $\epsilon$-attack accuracy of the network.
Given a network, an input $\vecx$, and an $\epsilon \geq 0$, the \emph{$\epsilon$-perturbation interval} $\perb{j}(\vecx)$ for each node $j$ in the network is defined recursively as follows:
%
\begin{itemize}

\item If $j$ is an input node with input value $x$, then $\perb{j}(\vecx) = [x - \epsilon, x+\epsilon]$ (intersected with any input constraints).

\item Otherwise, consider a node $q$ computing a function $f(\cdot)$ of its $n$ inputs, and let $\perb{1}(\vecx), \ldots, \perb{n}(\vecx)$ be the perturbation intervals of its inputs. 
Let ${\cali}^\epsilon(\vecx) = \prod_{1 \leq j \leq n} \perb{i}(\vecx)$ be the Cartesian product of the input intervals to the node, the perturbation interval of the node is then simply \\
$
    \perb{q}(\vecx) = 
    \Bigl[ 
        \min_{\vecz \in {\cali^\epsilon}(\vecx)} f(\vecz),
        \max_{\vecz \in {\cali^\epsilon}(\vecx)} f(\vecz)
    \Bigr]. 
$
\end{itemize}
%
The following theorem, provable by a simple induction on the network layers, states that the output of a network subject to input perturbations is always contained in the perturbation interval of its output. 

\begin{theorem}
If the network input $\vecx'$ is an $\epsilon$-perturbation of $\vecx$, then every node $j$ outputs values in its perturbation interval $\perbj(\vecx)$. 
\end{theorem}

The theorem, via the following corollary, yields a lower bound on a network's true $\epsilon$-attack accuracy.

\begin{corollary}
If the network predicts correctly on some test example $\vecx$ and every combination of values within the output nodes' $\epsilon$-perturbation intervals lead to the same prediction, then $\vecx$ has no $\epsilon$-adversary examples so $\vecx$ can be counted towards the network's true $\epsilon$-attack accuracy.

In particular, consider a classification problem with $n$ classes, and a classifier network $f$ with $n$ outputs, $y_1, \ldots, y_n$. 
Input $\vecx$ (belonging to, say, class 1) is classified correctly by $\vecy = f(\vecx)$ if $y_1 > y_k$ for $k = 2, \ldots, n$. 
To rule out the existence of $\epsilon$-attacks for $\vecx$, it suffices to check that $l_1 > r_k$ for $k = 2, \ldots, n$, where $[l_k, r_k] = {\cali}_k^\epsilon(\vecx)$ is the $\epsilon$-perturbation interval for output $k = 1, \ldots, n$ and input vector $\vecx$.
\end{corollary}

For many node types the perturbation intervals are easy to compute. 
In particular, for an MWD node, let $[l_1, r_1], \ldots, [l_n, r_n]$ be the perturbation intervals of its $n$ inputs for a given $\vecx$, and denote by $f(\cdot)$ the node function, defined as by (\ref{eq-rbf}).
Its output perturbation interval $[l, r]$ for $\vecx$ can be computed via 
$l = \max_{1 \leq i \leq n} \min \bigl\{ f(l_i), f(r_i) \bigr\}$, and  
$r = \max_{1 \leq i \leq n} m_i$,
where
\[
  m_i = 
  \begin{cases}
    1 & \mbox{if $l_i \leq w_i \leq r_i$} \\
    \max \bigl\{ f(l_i), f(r_i) \bigr\} & \mbox{otherwise.} 
  \end{cases}
\]
Computing these input-dependent perturbation intervals takes effort comparable to (perhaps 2$\times$ or 3$\times$) that of calculating the network's output.
Utilizing symbolic calculations, one could also calculate perturbation intervals as a function of the perturbation size $\epsilon$.



==> bounds_old.tex <==

This happens when, for example, the maximum of a node's perturbation interval requires minimizing one input while maximizing another.  
If no single perturbation of the network input simultaneously maximizes the first input and minimizes the other, then the maximum
of that node's perturbation interval cannot be achieved with an $\epsilon$-perturbation of the input.
Although perturbation intervals provide a safety guarantee, having a different classification result from using values in the output nodes' perturbation intervals does not 
imply the existence of an  $\epsilon$-adversarial example. 

\mynote{put theorem here}


A simple induction over the network's layers proves the following theorem.

\begin{theorem}
If the network input $\vecx'$ is an $\epsilon$-perturbation of $\vecx$, then every node $j$ outputs values 
in its perturbation interval $\perbj(\vecx)$. 
\end{theorem}

This shows that the perturbation intervals are \emph{safe} in the sense that \emph{every} $\epsilon$-perturbation of the 
input causes nodes to produce values in their perturbation intervals. 
Only when the perturbation intervals at the network's outputs are large enough to change the classification for input $\vecx$, can $\vecx$ have an $\epsilon$-adversary example.
This gives the following corollary showing that one can lower bound a network's true $\epsilon$-attack accuracy using the perturbation intervals for the test examples.

\begin{corollary}
If the network predicts correctly on some test example $\vecx$ and every combination of values within the output nodes' perturbation intervals lead to the same prediction, then 
$\vecx$ has no $\epsilon$-adversary examples so $\vecx$ can be counted towards the network's true $\epsilon$-attack accuracy.
\end{corollary}

Unfortunately, the perturbation intervals can over-estimate the amount of change an adversary can force.
This happens when, for example, the maximum of a node's perturbation interval requires minimizing one input while maximizing another.  
If no single perturbation of the network input simultaneously maximizes the first input and minimizes the other, then the maximum
of that node's perturbation interval cannot be achieved with an $\epsilon$-perturbation of the input.
Although perturbation intervals provide a safety guarantee, having a different classification result from using values in the output nodes' perturbation intervals does not 
imply the existence of an  $\epsilon$-adversarial example. 

In the supplementary materials we use a reduction from 3-SAT to prove the following theorem showing that it is difficult to determine if an endpoint of a perturbation interval can be achieved
by an $\epsilon$-perturbation.

\begin{theorem}
\label{t-np}
For every positive $\epsilon < 0.5$, there is a reduction from 3-SAT to a MWD network with a single output node such that on input $(1/2, \ldots, 1/2)$:
\begin{itemize}
\item The perturbation interval for the output node is $\left[e^{- \left(1- e^{-(2-(1/e))^2} \right)^2 }   , 1 \right] \approx [0.42, 1]$.
\item If the 3-SAT formula is satisfiable, then any output in the perturbation interval can be produced by an $\epsilon$-perturbation.
\item If the 3-SAT formula is not satisfiable, then no $\epsilon$-perturbation causes an output greater than 0.6.
\end{itemize}
Thus deciding even if the midpoint of a perturbation interval can produced by an $\epsilon$-perturbation is NP-complete.
\end{theorem}

This theorem shows that, in a sense, the one-sided perturbation interval guarantees are the best that can be produced by efficient algorithms.  
Despite this NP-completeness result, the perturbation intervals give sufficient information in enough cases to provide useful bounds
on the networks true $\epsilon$-attack accuracy, as the results section shows.
The ideas behind the reduction are easily generalized to other node types like ReLUs, giving analogous hardness results.


\subsection{NP-completeness - to be moved to supplementary materials}

In the following we sketch why determining whether or not a perturbation interval's endpoint can be achieved by an $\epsilon$-perturbation is NP-complete.

Recall Theorem~\ref{t-np}:
\begin{quote}
Given an MWD Network, a node $j$, an input $\vecx$, and an $\epsilon$, 
deciding if any $\epsilon$-perturbation of $\vecx$ causes node $j$ to output the maximum of its perturbation interval $S_j^\epsilon(\vecx)$ is NP-complete.
\end{quote}

The proof is by reduction from 3-SAT.  Recall that a 3-SAT instance consists of a set of boolean variables $V = \{v_1, \ldots, v_{|V|}\}$
and a set of clauses $C = \{c_1, \ldots, c_{|C|} \}$ where each $c_i$ consists of three literals and each literal is either some variable $v_j$ or its negation $\bar v_j$.
A clause is true if at least one of the literals in the clause is true, and the instance is satisfiable if there is a mapping of the variables to true/false making all of the clauses true.
We now assume w.l.o.g.~that no clause contains both a variable and its negation (it there were such a clause, it would always be true, and thus can be deleted from $C$ without affecting the
satisfiability of the instance).

We first show how to construct a corresponding MWD network and input from any 3-SAT instance.  For the construction, $\epsilon$ can be set to be any positive constant less than $0.5$.

The input nodes of the MWD network correspond to the variables, each input node $i$ corresponds to $v_i$ and each input value $x_i$ is set to $0.5$.
Increasing the value of the $x_i$ to $0.5+\epsilon$ corresponds to setting the variable to true, and decreasing its value to $0.5-\epsilon$ corresponds to setting it to false.

The first hidden layer has one node per literal that outputs a large value if the corresponding literal is made true by the perturbation, and a small value if it is made false.
Using MWD nodes, the node $j$ corresponding to literal $v_i$ has $u_{j,i}= 1/\epsilon$ and $w_{j,i} = 0.5+\epsilon$, with the other $u_{j,k}=0$.
This makes node $j$'s output  $\exp ( - \max (u_{j,i} (x_i - w_{j,i}) ) ) = 1$ if $x_i$ is perturbed to $0.5+\epsilon$ and less than $e^{-1}$ if $x_i$ is perturbed to 0.5 or less.
Similarly, the node $j$ corresponding to $\bar{v_i}$ 
has $u_{j,i} = 1/\epsilon$ and $w_{j_i} = 0.5-\epsilon$, so it produces 1 if $x_i$ is perturbed to $0.5-\epsilon$ and is less than $e^{-1}$ if $x_i$ is perturbed upwards.

The second hidden layer has one node per clause.
Consider a node $j$ corresponding to clause ($\ell_1$, $\ell_2$, $\ell_3$),  and let $i_1$, $i_2$, and $i_3$ be the nodes in the previous layer corresponding to the three literals.
The $u_{j,i}$ values will be 0 unless $i$ is in $\{i_1, i_2, i_3\}$ when $u_{j,i} = 2$. 
The $w_{j,i}$ values are all $e^{-1}/2$ (although only those for $i_1$, $i_2$, and $i_3$ are relevant).
Now the node $j$ will produce $e^{-(2-1/e)^2} < e^{-2.6}$ if any of ``its'' literals are ``true" 
and a value greater than $e^{-(1/e)^2} > 0.87 $ if all three associated variables were perturbed in the ``wrong'' direction.  

The output node takes as input each of the nodes on the second hidden layer.
Each $u$-value for the output node is 1, and each $w$-value  is $e^{-(2-1/e)^2}$.
Therefore, if each clause node has a ``true" literal then it outputs 1.
If any clause has all of its associated variables perturbed in the wrong direction then
the input from that clause's node is at least $0.87$, and 
output is at most $e^{-(0.87 - e^{-(2-1/e)^2})^2}  < 0.6$.

By the construction, if the 3-sat formula is satisfiable, then any $\epsilon$-perturbation of the input $(1/2, \ldots, 1/2)$ corresponding to a satisfying truth assignment achieves an output of 1.
Conversely, if some $\epsilon$-perturbation achieves an output greater than 0.6, then the inputs are perturbed in a way so that every clause-node has 
at least one of its literal-node inputs perturbed towards true.  Thus the perturbation directions of the inputs can be used to create satisfying truth assignment.

For the constructed network, the perturbation intervals of the nodes corresponding to literals are $[e^{-2}, 1]$,
the perturbation intervals for the nodes corresponding to clauses are $[e^{-(2-(1/e))^2}, 1]$.
and the perturbation interval for the output node is $\left[e^{- \left(1- e^{-(2-(1/e))^2} \right)^2 }   , 1 \right] \subset [0.4 ,1]$.

Note that, assuming the 3-SAT formula is satisfiable and not a tautology, there are $\epsilon$-perturbations producing both end points of the output node's 
perturbation interval.  
Since the network output is a continuous function of its inputs, this means that every out value in the perturbation interval can be produced by some $\epsilon$-perturbation.
On the other hand, if the 3-SAT formula is not satisfiable then no $\epsilon$-perturbation can cause an output above 0.6, so more than the top half of the output node's perturbation interval
cannot be achieved by $\epsilon$-perturbations.

Thus determining if any $\epsilon$-perturbation causes the output node to produce a value in the top half of its perturbation interval NP-complete problem.

The preceding proof exploited the $\max$ in the MWD nodes to simulate a satisfiability instance.  
The non-linearity in ReLUs can used to simulate satisfiability in a similar construction,
so that determining if the top part of an output node's perturbation interval is achievable by an $\epsilon$-perturbation is
also NP-complete for ReLU networks.

\textbf{Note: following table for ease of checking proof, see also \texttt{NP proof calc.ipynb} }

\begin{tabular}{c c c c c c}
node    & u         &  w    & min               & mid           &  max \\
inp/var     & --        & --            & $0.5-\epsilon$    & 0.5           & $0.5+\epsilon$ \\
literal  & $1/\epsilon$ & $0.5 \pm \epsilon$ & $e^{-2}$  &  $e^{-1}$    & 1 (true) \\
clause   & 2        & $ e^{-1}/2$ &  $e^{-(2-e^{-1})^2}$ & $e^{-(e^{-1})^2} $    & 1 (??) \\
output  & 1     & $e^{-(2-1/e)^2}$ &     $e^{-(1-w)^2}  $   &  ??               & 1 (true) \\
output  &       &  &    $\displaystyle e^{-(1- e^{-(2-1/e)^2})^2} $ 
\end{tabular}



==> experiments.tex <==
\section{Experimental Setup}

%\ificlrfinal
%We implemented \rbfinf\ networks in the PyTorch framework (\cite{PaszkeAutomaticdifferentiationpytorch2017}); the implementation is available at \url{\codeurl}.
%\else
We implemented \rbfinf\ networks in the PyTorch framework (\cite{PaszkeAutomaticdifferentiationpytorch2017}).
%\fi
In order to extend PyTorch with a new function $f$, it is necessary to specify the function behavior $f(\vecx)$, and the function gradient $\grad_{\vecx} f$.
To implement \rbfinf, we extend PyTorch with two new functions: a {\em LargeAttractorExp\/} function, with forward behavior $e^{-x}$ and backward gradient propagation according to $-1/\sqrt{1 + x}$, and {\em SharedFeedbackMax,} with forward behavior $y = \max_{i=1}^n x_i$ and backward gradient propagation according to $e^{x_i - y}$. 
These two functions are used in the definition of \rbfinf\ units, as per (\ref{eq-rbfinf}), with the AutoGrad mechanism of PyTorch providing  backward (pseudo)gradient propagation for the complete networks.

% We also introduced to PyTorch {\em bounded parameters,} which have a prescribed range that is enforced during network training; these bounded parameters were used to implement our $\vecu$ and $\vecw$ weight vectors. 

\paragraph{Dataset.}
We use the MNIST dataset (\cite{LeCunGradientbasedlearningapplied1998}) for our experiments, following the standard setup of 60,000 training examples and 10,000 testing examples. 
Each digit image was flattened to a one-dimensional feature vector of length $28 \times 28 = 784$, and fed to a fully-connected neural network; this is the so-called {\em permutation-invariant\/} MNIST. 

\paragraph{Neural networks.}
We compared the accuracy of the following fully-connected network structures. 
%
\begin{itemize}

\item {\bf ReLU} networks (\cite{NairRectifiedlinearunits2010}) whose output is fed into a softmax, and the network is trained via cross-entropy loss. 

\item {\bf Sigmoid} networks trained with square-error loss. 

\item {\bf \rbfinf}
networks, trained using square-error loss. 
For a \rbfinf\ network with $m$ layers, we denote its type as $\rbfnet(K_1, \ldots, K_m \mid t_1, \ldots, t_m)$, where $K_1, \ldots, K_m$ are the numbers of units in each layer, and where the units in layer $i$ are And units if $t_i = \und$, Or units if $t_i = \oder$, and are a random mix of And and Or units if $t_m = \ast$. 

\end{itemize}
%
Square-error loss worked as well or better than other loss functions for Sigmoid and RBFI networks.
Unless otherwise noted, we use networks with layers 512, 512, 512, and 10 units, and in case of RBFI networks, we used geometry $\rbfnet(512, 512, 512, 10 \mid \und, \oder, \und, \oder)$.
For RBFI networks we use a bound of $[0.01, 3]$ for the components of the $u$-vectors, and of $[0, 1]$ for the $w$-vectors, the latter corresponding to the value range of MNIST pixels. 
We experimented with RBFI networks with various geometries, and we found the performance differences to be rather small.
We trained all networks with the AdaDelta optimizer (\cite{ZeilerADADELTAadaptivelearning2012}), which yielded good results for all networks considered.  
% When reporting an accuracy as $X\% \pm Y\%$, $X$ is the mean value of the percent accuracy, and $Y$ the standard deviation of the individual run outcomes.
% Error bars in the plots correspond to one standard deviation of individual run results.

\paragraph{Attacks.}
We applied FGSM, I-FGSM, and noise attacks to the whole test set.
In I-FGSM attacks, we performed 10 iterations of (\ref{eq-I-FGSM}).  
As PGD attacks are computationally intensive, we apply them to one run only, and we compute the performance under PGD attacks for the first 5,000 examples in the test set only.
For each input $\vecx$ in the test set, we perform 20 PGD searches, or restarts.
In each search, we start from a random point in $\ball_\epsilon(\vecx)$ and we perform 100 steps of projected gradient descent using the AdaDelta algorithm to tune step size; if at any step a misclassified example is generated, the attack is considered successful. 

For \rbfinf\ networks, we can perform FGSM, I-FGSM, and PGD attacks based either on true gradient, or on the pseudogradients. 
We denote the pseudogradient-based attacks as FGSM[psd], I-FGSM[psd], and PGD[psd], respectively. 
Such attacks in general are more powerful than attacks based on the regular gradient, for the same reason why the pseudogradient is more effective in training.



